MD-Bench: A generic proxy-app toolbox for state-of-the-art molecular dynamics algorithms

Proxy-apps, or mini-apps, are simple self-contained benchmark codes with performance-relevant kernels extracted from real applications. Initially used to facilitate software-hardware co-design, they are a crucial ingredient for serious performance engineering, especially when dealing with large-scale production codes. MD-Bench is a new proxy-app in the area of classical short-range molecular dynamics. In contrast to existing proxy-apps in MD (e.g. miniMD and coMD) it does not resemble a single application code, but implements state-of-the art algorithms from multiple applications (currently LAMMPS and GROMACS). The MD-Bench source code is understandable, extensible and suited for teaching, benchmarking and researching MD algorithms. Primary design goals are transparency and simplicity, a developer is able to tinker with the source code down to the assembly level. This paper introduces MD-Bench, explains its design and structure, covers implemented optimization variants, and illustrates its usage on three examples.

==> latexmkrc <==
# `-file-line-error` is similar to `--interaction nonstopmode`, but shows the concrete line number
# Remove it, it you want lualatex to stop on errors
$pdflatex = 'pdflatex --shell-escape --interaction nonstopmode --synctex=-1 %O %S ';

#Use SumatraPDF instead of the default PDF viewer
$pdf_previewer = 'start "C:\Program Files\SumatraPDF\SumatraPDF.exe"';

#SumatraPDF updates automatically
$preview_mode = 0;

#automatically call lualatex/pdflatex (instead of latex)
$pdf_mode = 1;

add_cus_dep('glo', 'gls', 0, 'run_makeglossaries');
add_cus_dep('acn', 'acr', 0, 'run_makeglossaries');

sub run_makeglossaries {
  if ( $silent ) {
    system "makeglossaries", "-q", $_[0];
  }
  else {
    system "makeglossaries", $_[0];
  };
}

# enable deletion of *.bbl when calling "latexmk -c"
$bibtex_use = 2;

#remove more files than in the default configuration
@generated_exts = qw(acn acr alg aux code ist fls glg glo gls glsdefs idx ind lof lot out thm toc tpt wrt upa upb synctex);
$clean_ext .= ' %R.ist %R.xdy';

